Classical and Quantum Thermodynamic Systems in Curved Spacetime

Systems at finite temperature make up the vast majority of realistic physical scenarios. Indeed, although zero temperature is often accompanied by simpler mathematics, the richness in physical results is evident when one considers the system to have temperature and even more so if the background geometry is curved. This thesis will be dedicated to the study of this type of physical systems, where thermodynamics and general relativity equally contribute to the dynamics. The first part will be devoted to the study of classical thermodynamic systems in curved spacetime, namely thin matter shells at finite temperature. These objects partition spacetime into separate pieces, and their very existence is conditioned by the so-called junctions conditions. The latter conditions allow us to carefully study both the mechanical and thermodynamics of the shell and, in particular, they give rise to a well-defined notion of entropy. The shell can then be taken to its black hole limit, providing an alternative way to study black hole thermodynamics. We will do this for different geometries, obtaining as byproduct a plausible answer for the debated value of the entropy of an extremal black hole. In the second part we shall review the standard formalisms to study QFT in curved spacetimes, in order to explore quantum properties of thermodynamic systems in the presence of gravity. Massive quantum scalar fields at finite temperature will be the systems of choice, whereby various instances of vacuum polarisation will be calculated in a variety of black hole geometries. Both numerical and analytic results will be obtained, and new addition formulas for a certain class of transcendental functions will be derived. This part will culminate with a careful numerical study of symmetry restoration of a self-interacting scalar field around a charged black hole, where we verify insights present in the literature.

==> 2.citation.tex <==
\thispagestyle{empty}
\hbox{} \vfill
\begin{flushright}
\small \textit{\textbf{Bitches be crazy.}}
\\ \vspace{2mm}
\scriptsize Dalai Lama
\end{flushright}

\clearpage
\thispagestyle{empty}
\cleardoublepage

==> I.3ShellCharged/5.section.tex <==
\section{The thin shell and the black hole limit}
\label{bhlimit}



Let us consider a charged thin shell, for which the differential of
the entropy has been deduced to be Eq.~(\ref{dSQ}).
We are free
to choose an equation of state for the inverse temperature.
Let us pick for convenience the following inverse temperature
dependence,
\begin{equation}\label{bBH}
b(r_+,r_-) = \gamma\,
\frac{r_+^2}{r_+-r_-}\,,
\end{equation}
where $\gamma$ is some constant with
units of inverse mass times inverse radius,
i.e., units of angular momentum.




For a charged shell we must also specify the function $c(r_+,r_-)$,
whose form can be taken from
the differential equation (\ref{bc5}) upon
substitution of the function (\ref{bBH}).
There is a family of solutions
for $c(r_+,r_-)$
but for
our purposes here we choose
the following specific solution,
\begin{equation}\label{cBH}
c(r_+,r_-) = \frac{1}{r_+}\,.
\end{equation}
The reason for the choices above becomes clear when
we discuss the shell's gravitational radius, i.e., black hole
limit.
Inserting the choice for $b(r_+,r_-)$, Eq.~(\ref{bBH}),
along with the  choice for the function
$c(r_+,r_-)$,  Eq.~(\ref{cBH}), in the
differential (\ref{dSQ}) and integrating, we obtain the entropy
differential for the
shell
\begin{equation}\label{diffSS}
dS = \frac{\gamma}{2\, G} \,r_+\, dr_+\,.
\end{equation}
Thus, the entropy of the shell is
$S=\frac{\gamma}{4\, G} \,r_+^2+ S_0$,
where $S_0$ is an integration constant.
Imposing that when the shell vanishes
(i.e., $M=0$ and $Q=0$, and so
$r_+=0$) the entropy vanishes,
we have that $S_0$ is zero,
and so
$S=\frac{\gamma}{4\, G} \,r_+^2$.
Thus, we can write
the entropy $S(M,R,Q)$ as
\begin{equation}\label{SSa}
S = \frac{\gamma}{16\pi G}\, A_+\,,
\end{equation}
where $A_+$ is the gravitational
area of the shell, as given in
Eq.~(\ref{areaplus}).
This result shows that the entropy of this thin
charged shell
depends on $(M,R,Q)$ through
$r_+^2$ only, which itself is
a specific function of $(M,R,Q)$.





Now, the constant $\g$ should be determined
by the properties of the matter in the shell,
and cannot be decided a priori. The thermodynamic stability of the uncharged case ($Q=0$, i.e.,
$r_-=0$) can be worked out
\cite{Martinez:1996ni} and elucidates the issue.  In the
uncharged case the nontrivial stability conditions are given by
Eqs.~(\ref{B1}) and (\ref{B4}).
Equation~(\ref{B1}) gives immediately
$R\leq\frac32 r_+$, i.e., $R\leq3Gm$. On the other hand,
Eq.~(\ref{B4}) yields $R\geq r_+$, i.e., $R\geq2Gm$. Thus, the
stability conditions yield the following range for $R$, $r_+\leq
R\leq\frac32 r_+$, or in terms of $m$, $2Gm\leq R\leq 3Gm$. This is
precisely the range for stability found by York \cite{York:1986it} for a
black hole in a canonical ensemble in which a spherical massless thin
wall at radius $R$ is maintained at fixed temperature $T$. In
\cite{York:1986it} the criterion used for stability is that the heat
capacity of the system should be positive, and physically such a tight
range for $R$ means that only when the shell, at a given temperature
$T$, is sufficiently close to the horizon can it smother the
black hole enough
to make it thermodynamically stable. The positivity of the heat
capacity is equivalent to our stability conditions, Eqs.~(\ref{B1})
and (\ref{B4}) in the uncharged case.

The stability conditions, Eqs.~(\ref{B1})-(\ref{B7}), for the general
charged case cannot be solved analytically in this instance, they
require numerical work, which will shadow what we want to
determine. Nevertheless, the approach followed in
\cite{Braden:1990hw,Peca:1998cs} for the heat capacity of a charged black
hole in a grand canonical ensemble gives a hint of the procedure that
should be followed.



Although $\gamma$ should be determined
by the properties of the matter in the shell,
there is a case in which the properties
of the shell have to adjust to the
environmental properties of the spacetime.
This is the case when
$R
\to r_+$.
In this case, one must note that, as the shell approaches its own
gravitational radius, quantum fields are inevitably present and their
backreaction will diverge unless we choose the
black hole Hawking temperature
$T_{\rm bh}$
for the temperature of the shell (citar formula de D dimensoes).
In this case, $R\to r_+$,
we must take the temperature of
the shell as
$T_{\rm bh} = \frac{\hbar}{4 \pi} \frac{r_+-r_-}{r_+^2}$,
where $\hbar$ is Planck's constant.
So we must choose
\begin{equation}
\gamma= \frac{4\pi}{\hbar} \,,
\label{ga}
\end{equation}
i.e., $\gamma$ depends on fundamental constants.
Then,
\begin{equation}\label{thawk}
b(r_+,r_-) = \frac{1}{T_{\rm bh}}
=\frac{4 \pi} {\hbar}
\frac{r_+^2}{r_+-r_-}\,.
\end{equation}
In this case the entropy of the shell is
$S= \frac14\frac{A_+}{G\hbar}$, i.e.,
\begin{equation}\label{SS}
S=
\frac{1}{4}\frac{A_+}{A_p}\,,
\end{equation}
where $l_p=\sqrt{G\hbar}$ is the Planck length, and $A_p=l_p^2$ the
Planck area.
Note now that the entropy
given in Eq.~(\ref{SS})
is the black hole Bekenstein-Hawking entropy
$S_{\rm bh}$ of a charged black hole since
\begin{equation}\label{SSBH}
S_{\rm bh}= \frac{1}{4}\frac{A_+}{A_p}\,,
\end{equation}
where $A_+$ is here the horizon area.  Thus, when we
take the shell to its own gravitational radius the entropy is the
Bekenstein-Hawking entropy.  The limit also implies that the pressure
and the thermodynamic electric potential go to infinity as $1/k$,
according to Eqs.~(\ref{pQk}) and (\ref{Phi}), respectively.  Note,
however, that the local inverse temperature goes to zero as $k$, see
Eq.~(\ref{BS5}), and so the local temperature of the shell also goes
to infinity as $1/k$. These well-controlled infinities cancel out
precisely to give the Bekenstein-Hawking entropy (\ref{SS}).


Note that the shell at its own gravitational radius, at least in
the uncharged case, is thermodynamically stable, since in this case
stability requires $r_+\leq R\leq\frac32 r_+$, as mentioned above. In
addition, our approach and the approach followed in
\cite{Pretorius:1997wr} to find the black hole entropy have some
similarities. The two approaches use matter fields, i.e., shells,
to find the black hole entropy. Here we use a static shell
that decreases its own radius $R$ by steps, maintaining its staticity
at each step. In \cite{Pretorius:1997wr} a reversible contraction of a thin
spherical shell down to its own gravitational radius was examined, and
it was found that the black hole entropy can be defined as the
thermodynamic entropy stored in the matter in the situation that the
matter is compressed into a thin layer at its own gravitational
radius.



Finally we note that the extremal limit $\sqrt{G}m=Q$ or $r_+=r_-$
is well defined from above.  Indeed, when one takes the limit $r_+\to
r_-$ one finds that $1/b(r_+,r_-)=0$ (i.e., the Hawking temperature is
zero) and the entropy of the extremal black hole is still given by
$S_{\rm extremal\,bh}= \frac{1}{4}\frac{A_+}{A_p}$.  It is well known
that extremal black holes and in particular their entropy have to be
dealt with care.  If, ab initio, one starts with the analysis for an
extremal black hole one finds that the entropy of the extremal black
hole has a more general expression than simply being equal to one
quarter of the area \cite{Pretorius:1997wr,Lemos:2010kw}.  This
extremal shell is an example of a Majumdar-Papapetrou matter system.
Its pressure $p$ is zero, and it remains zero, and thus finite, even
when $R\to r_+$.  This limit of $R\to r_+$ is called a quasiblack
hole, which in the extremal case is a well-behaved one.

It is important to stress that the requirement $b=T_{\mathrm{bh}}^{-1}$
is compulsory
only for shells that approach their own gravitational
radius. Otherwise, if we consider the radius of the shell within some
constrained region outside the gravitational radius, the shell
temperature can be arbitrary since away from the horizon, quantum
backreaction remains modest and does not destroy the thermodynamic
state.
One can discuss whole classes of functions $b(r_{+},r_{-})\neq
T_{\mathrm{bh}}^{-1}$. The choice (\ref{cBH}) for $c$ is also only necessary
for shells at the gravitational radius limit.
According to Eq.~(\ref{cr+r-}), this gives us
$\phi =\frac{ \sqrt{r_-} }{ \sqrt{G\, r_{+} }}$, i.e.,
\begin{equation}
\phi =\frac{Q}{r_{+}}  \label{rn}
\end{equation}
that coincides with the standard expression for the electric potential
for the Reissner-Nordstr\"{o}m black hole. In addition,
Eq.~(\ref{Phi})
acquires the form
\begin{equation}
\Phi =\frac{Q}{k}\left(\frac{1}{r_{+}}-\frac{1}{R}\right)
\label{frn}
\end{equation}
that coincides entirely with the corresponding formula for the
Reissner-Nordstr\"{o}m black hole in
a grand canonical ensemble \cite{Braden:1990hw}.  Meanwhile, in this
case there is no black hole.  Moreover, considering the uncharged
case, $Q\rightarrow0$ or
$r_{-}\rightarrow 0$, it is seen from Eq.~(\ref{dSQ}) that the
quantity $c$ drops out from the entropy, so the choice of $c$ is
relevant for the charged case only.





There are similarities between the thin-shell approach and
the black hole mechanics approach \cite{Bardeen:1973gs}.
These are evident if we express the
differential of the entropy of the charged shell (\ref{dSQ}) in terms
of the black hole ADM
mass $m$ and charge $Q$, given in terms of the
variables $(r_+,r_-)$ by
Eqs.~(\ref{invhorradi})-(\ref{invhorradicauch}).
The differential for the entropy of the shell reads,
in these variables,
\begin{equation}
T_0 dS = dm - c\, Q\, dQ
\end{equation}
where we have defined $T_0 \equiv 1/b(r_+,r_-)$ which is the
temperature the shell would possess if located at infinity.
Here, $T_0 =1/b(r_+,r_-)$ and $c=c(r_+,r_-)$ should be seen as
$T_0 (m,Q)=1/b(m,Q)$ and $c(m,Q)$, respectively,
since $r_+$ and $r_-$ are functions of
$m$ and $Q$.
As we have
seen, if we take the shell to its gravitational radius, we must fix
$T_0 = T_{\rm bh}$ and $c = 1/r_+$.
This suggests that $Q/r_+$ should play the role of
the black hole electric potential $\Phi_{\rm bh}$, which in fact is
true, as shown in Eq.~(\ref{rn}).
This implies that the
conservation of energy of the shell is expressed as
\begin{equation}\label{1T7}
T_{\rm bh} dS_{\rm bh} = dm - \Phi_{\rm bh}\, dQ\,.
\end{equation}
We thus
see that the first law of thermodynamics for the shell
at its own gravitational radius is
equal to the energy conservation for the
Reissner-Nordstr\"om
black hole.



==> II.3BTZ/3.section.tex <==
\section{Regularization of the coincidence limit}

In the coincidence limite, the only term which automatically originates a divergence at every point in spacetime is the first term in the right hand side of Eq.~(\ref{nPQc}). Its regularisation has already been done in \cite{Shiraishi:1993nu}, but we will repeat it hre in a slightly different manner, in order to explicitely check that the counterterms must be of the form of Eq.~(\ref{GdivO}), derived in Chapter 8.








==> II.55Dcharged/4.section.tex <==
\section{Renormalization of the effective action}

As is well known in QFT, divergences appear when calculating quantum corrections to a wide variety of quantities, and the process to isolate and remove these divergences is know as renormalization. There is no unique way to renormalize a divergent quantity, but there are some procedures which work best under certain situations. The Schwinger approach to QFT allows us to formulate a rigorous way to do this in curved spacetime, by compacting all leading order corrections into a single quantity $\Gamma^{(1)}$, through the use of the heat kernel $K(\tau;x,x')$. The power of this method lies in the fact that the dynamics of the heat kernel is entirely characterized by Eq.~(\ref{SchroEq}), an equation which has been extensively scrutinized in the literature.

The renormalization of $\Gamma^{(1)}$ will be considered for differential operators of the form (leaving indexes implicit)
\eq{\label{OpeF}
\ma{F} = g^{\mu \nu} \nabla_{\mu} \nabla_{\nu} + Q(x)
}
where $\nabla_{\mu}$ is any covariant derivative (including gauge potentials or connections derived from spacetime curvature) and $Q(x)$ does not contain any derivatives with respect to spacetime indexes. The form considered in Eq.~(\ref{OpeF}) is actually one of the most general ones and all cases considered in this work will fall into that category. When one studies the flat spacetime limit of Eq.~(\ref{SchroEq}), it becomes evident that the divergent behavior comes from the integration in $\tau$. Since the heat kernel will always contain a negative imaginary part from the Feynman boundary conditions, i.e. from the substitution $m^2 \to m^2 - i\e$, it can be shown that the heat kernel is expected to decay exponentially fast for large values of $\tau$. This means the only possible source of divergences lies in the small $\tau$ regime, for which it is well know that the heat kernel posesses an expansion of the form
\eq{\label{smalltau}
K(\tau;x,x') \propto {i \over (4\pi i \tau)^{d/2}} \sum^{\infty}_{k=0} (i\tau)^k E_{k}(x)
}
where the first few coefficients $E_k(x)$ are given by
\ea{
E_0(x) & = I\,, \\
E_1(x) & = {1 \over 6} R I - Q\,, \\
E_2(x) & = \left( -{1\over 30} \square R + {1 \over 72} R^2 -{1\over 180} R^{\mu\nu}R_{\mu\nu} + {1\over 180} R^{\mu\nu\rho\si}R_{\mu\nu\rho\si}\right) I \nonumber \\
       & \hspace{5mm} + {1\over 12} W^{\mu\nu}W_{\mu\nu} + {1 \over 2} Q^2 - {1\over 6} R Q + {1\over 6}\square Q\,,
}
with
\eq{
W_{\mu\nu} = [\nabla_{\mu},\nabla_{\nu}]
}
and where $I$ denotes the identity in whatever indexes appear in the theory. Inserting the expansion (\ref{smalltau}) in Eq.~(\ref{G1func}), it becomes clear that the divergent part of $\Gamma^{(1)}$ is given by
\eq{
\textbf{divp} \, \Gamma^{(1)} = {i\over 2 (4\pi)^{d/2}} \int dv_x \sum^{\infty}_{k=0} \textrm{Tr} E_{k}(x) \, \textbf{divp} \int^{\tau_0}_{0} d\tau (i\tau)^{k-1-d/2}
}
where $\textbf{divp}$ denotes the divergent part and $\tau_0$ is a constant which we may take as small as we like. It remains to evaluate the integral in $\tau$, which gives
\eq{
\int^{\tau_0{\infty}}_{0} d\tau (i\tau)^{k-1-d/2} = (i)^{k-1-d/2} {\tau_0^{k-n/2} \over k-d/2}\,.
}
Evidently, for odd $d$ the integral will vanish when $\tau\to 0$, but it will diverge for $k=d/2$ and even $d$. One may isolate the divergences in many different ways and in this case we will employ the so-called dimensional regularization method, whereby one performs the substitution $d \to d+\e$, where $\e$ is some small quantity assumed to go to zero in the end. By doing this, we conclude that
\eq{
\textbf{divp} \int^{\tau_0{\infty}}_{0} d\tau (i\tau)^{k-1-d/2} = {2i \over \e}
}
which finally leads to the desired result
\eq{\label{divG1}
\textbf{divp} \, \Gamma^{(1)} = -{1\over \e(4\pi)^{d/2}} \int dv_x  \textrm{Tr} E_{d/2}(x)\,.
}
At leading-order, one must then guarantee that there are enough parameters in the action to compensate for the existence of the divergences given by Eq.~(\ref{divG1}). This procedure is not suitable for odd dimensionality, but will only make use of these results for even dimensions in this work.
